From Attention to Activation: Unravelling the Enigmas of Large Language Models

We study two strange phenomena in auto-regressive Transformers: (1) the dominance of the first token in attention heads; (2) the occurrence of large outlier activations in the hidden states. We find that popular large language models, such as Llama attend maximally to the first token in 98% of attention heads, a behaviour we attribute to the softmax function. To mitigate this issue, we propose a reformulation of softmax to softmax-1. Furthermore, we identify adaptive optimisers, e.g. Adam, as the primary contributor to the large outlier activations and introduce OrthoAdam, a novel optimiser that utilises orthogonal matrices to transform gradients, to address this issue. Finally, not only do our methods prevent these phenomena from occurring, but additionally, they enable Transformers to sustain their performance when quantised using basic algorithms, something that standard methods are unable to do. In summary, our methods reduce the attention proportion on the first token from 65% to 3.3%, the activation kurtosis in the hidden states from 1657 to 3.1, and perplexity penalty under 4-bit weight quantisation from 3565 to 0.3.

==> assets/figures/causal_figure_red.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
    \centering
    \footnotesize
    \includegraphics[width=0.4\textwidth]{assets/figures/paper_figures/causal_model_attn_red.eps}
    \caption{Blah blah}\label{fig:causal}
\end{wrapfigure}

==> assets/figures/teaser_figure_red_red.tex <==
\begin{figure}
    \centering
    \footnotesize
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{assets/figures/paper_figures/reference_model_attn_red.eps}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.75\textwidth}
        \includegraphics[width=\textwidth]{assets/figures/paper_figures/reference_model_hs_red.eps}
    \end{minipage}
\end{figure}
\begin{figure}
    \vspace{-0.5cm}
    \centering
    \footnotesize
    \begin{minipage}[t]{0.24\textwidth}
        \includegraphics[width=\textwidth]{assets/figures/paper_figures/our_model_attn_red.eps}\label{fig:image1}
        \subcaption{}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.75\textwidth}
        \includegraphics[width=\textwidth]{assets/figures/paper_figures/our_model_hs_red.eps}\label{fig:image2}
        \subcaption{}
    \end{minipage}
    \caption{Blah blah}\label{fig:sidebyside}
\end{figure}

==> assets/tables/main_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[!t]
    \begin{adjustbox}{width=\linewidth}
    \begin{tabular}{c|c|cc|c|cc|cc|cc}
    \toprule
    \multirow{2}{*}{Model}  & \multirow{2}{*}{\#Parameters} & \multirow{2}{*}{Softmax+1?} & \multirow{2}{*}{OrthoAdam?} & \multirow{2}{*}{PPL} & \multicolumn{2}{c|}{Mean Layer Kurtosis} & \multicolumn{2}{c|}{Median Layer Kurtosis} & \multicolumn{2}{c}{Max Absolute Activation} \\
                            &                               &                             &                             &                      & First Token        & Other Tokens        & First Token         & Other Tokens         & First Token          & Other Tokens         \\ \midrule
    \multirow{12}{*}{GPT2*} & \multirow{4}{*}{60M}          &                             &                             & xx.yy                & xxx                & xxx                 & xxx                 & xxx                  & xxxx                 & xxxx                 \\
                            &                               & \checkmark                  &                             & xx.yy                & xxx                & xxx                 & xxx                 & xxx                  & xxxx                 & xxxx                 \\
                            &                               &                             & \checkmark                  & xx.yy                & xxx                & xxx                 & xxx                 & xxx                  & xxxx                 & xxxx                 \\
                            &                               & \checkmark                  & \checkmark                  & xx.yy                & xxx                & xxx                 & xxx                 & xxx                  & xxxx                 & xxxx                 \\ \cmidrule(l){2-11} 
                            & \multirow{4}{*}{130M}         &                             &                             & xx.yy                & xxx                & xxx                 & xxx                 & xxx                  & xxxx                 & xxxx                 \\
                            &                               & \checkmark                  &                             & xx.yy                & xxx                & xxx                 & xxx                 & xxx                  & xxxx                 & xxxx                 \\
                            &                               &                             & \checkmark                  & xx.yy                & xxx                & xxx                 & xxx                 & xxx                  & xxxx                 & xxxx                 \\
                            &                               & \checkmark                  & \checkmark                  & xx.yy                & xxx                & xxx                 & xxx                 & xxx                  & xxxx                 & xxxx                 \\ \cmidrule(l){2-11} 
                            & \multirow{2}{*}{350M}         &                             &                             & xx.yy                & xxx                & xxx                 & xxx                 & xxx                  & xxxx                 & xxxx                 \\
                            &                               & \checkmark                  & \checkmark                  & xx.yy                & xxx                & xxx                 & xxx                 & xxx                  & xxxx                 & xxxx                 \\ \cmidrule(l){2-11} 
                            & \multirow{2}{*}{1.4B}         &                             &                             & xx.yy                & xxx                & xxx                 & xxx                 & xxx                  & xxxx                 & xxxx                 \\
                            &                               & \checkmark                  & \checkmark                  & xx.yy                & xxx                & xxx                 & xxx                 & xxx                  & xxxx                 & xxxx                 \\ \midrule
    \multirow{4}{*}{Llama2} & \multirow{4}{*}{130M}         &                             &                             & xx.yy                & xxx                & xxx                 & xxx                 & xxx                  & xxxx                 & xxxx                 \\
                            &                               & \checkmark                  &                             & xx.yy                & xxx                & xxx                 & xxx                 & xxx                  & xxxx                 & xxxx                 \\
                            &                               &                             & \checkmark                  & xx.yy                & xxx                & xxx                 & xxx                 & xxx                  & xxxx                 & xxxx                 \\
                            &                               & \checkmark                  & \checkmark                  & xx.yy                & xxx                & xxx                 & xxx                 & xxx                  & xxxx                 & xxxx                 \\ \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table}

==> assets/tables/teaser.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[h!]
    \begin{adjustbox}{width=\linewidth}
    \begin{tabular}{l|c|cc|c|c|c}
    \toprule
    \multirow{2}{*}{Model} & \multirow{2}{*}{\#Parameters} & \multicolumn{2}{c|}{PPL}   & \multirow{2}{*}{Max Absolute Activation}    & \multirow{2}{*}{Activation Kurtosis} & \multirow{2}{*}{Max Attended First Token} \\
                           &                               & FP16    & 4-bit Quant      &                                             &                                      &                                           \\ \midrule
    GPT2-Small             & 137M                          & 37.8    &   4456.1         & xxxx                                        & xxxx                                 & 0.73                                      \\
    GPT2-Medium            & 350M                          & 28.8    &   2435.3         & xxxx                                        & xxxx                                 & 0.76                                      \\
    GPT2-Large             & 812M                          & 25.2    &    571.0         & xxxx                                        & xxxx                                 & 0.68                                      \\
    GPT2-XL                & 1.6B                          & 23.2    &   7981.8         & xxxx                                        & xxxx                                 & 0.51                                      \\ \midrule
    Llama2-7B              & 6.7B                          &  7.7    & 191477.5         & xxxx                                        & xxxx                                 & 0.80                                      \\
    Llama3.1-8B            & 8B                            & 10.2    &   xxxx.y         & xxxx                                        & xxxx                                 & 0.95                                      \\ \midrule
    \rowcolor[HTML]{C0C0C0}
    GPT2 (Ours)            & 350M                          & 16.3    &     17.1         & xxxx                                        & xxxx                                 & x.yy                                      \\ 
    \rowcolor[HTML]{C0C0C0}
    GPT2 (Ours)            & 1.4B                          & xx.y    &   xxxx.y         & xxxx                                        & xxxx                                 & x.yy                                      \\ \bottomrule
    \end{tabular}
    \end{adjustbox}
\end{table}

==> sections/04-sm1.tex <==
\section{Method: First Token Domination}\label{sec:meth-first-token}
In this section we shall eliminate certain plausible causes of the two anomalies in transformer models.
We shall primarily consider GPT2 as a representative transformer model, due to its simplicity,
but also consider Llama models to narrow down the potential causes of the anomalies.
In all our experiments, unless stated otherwise, we use a GPT2 model with $\sim$130M parameters
trained on the \texttt{en} split of the C4 dataset.
The various changes we make to the model are described throughout the paper
as we eliminate potential causes of the anomalies. 

\subsection{Eliminating Certain Causes}\label{ssec:elim-first-token}
Given that GPT2 models and Llama models both exhibit the first token dominance in attention maps,
we only consider the parts of the transformer architecture that are common to both models
as potential causes of this anomaly.
GPT2 and Llama architectures differ in the following aspects:
% reduce spacing before itemize
\begin{itemize}[noitemsep,topsep=0pt]
    \setlength\itemsep{0em} % reduce itemize spacing
    \item Llama models use Rotary Positional Encodings (RoPE)~\citep{su2024roformer}, while GPT2 models uses learnt absolute positional encodings~\citep{vaswani2017attention}.
    \item Llama models use a \texttt{<bos>} token to denote the beginning of a sequence, while GPT2 models do not.
    \item Llama models use SiLU~\citep{elfwing2018sigmoid} activations in the feedforward layers, while GPT2 models use GeLU activations~\citep{hendrycks2016gaussian}.
    \item Llama models use RMSNorm~\citep{zhang2019root} as the normalisation layer, while GPT2 models use LayerNorm~\citep{ba2016layer}.
\end{itemize}
Although, Llama and GPT2 use different kinds of positional encodings, they both do use some kind of positional encodings.
Therefore it is plausible that the positional encodings privilege the first token in a way
that leads to the first token dominance in attention maps.
The remaining differences between the two models listed above do not affect the first token differently
compared to other tokens~\ie~the normalisation layer and the activation function are applied identically to all token positions.
Therefore, we train a GPT2 model \emph{without any positional encodings} and observe the attention maps,
comparing them to another GPT2 model trained with learnt absolute positional encodings, all other parameters and hyperparameters being the same.

We find the GPT2 model without (with) positional encodings
exhibits first token dominance in 33\% (20\%) of the (query, head) pairs and
allocates 17\% (10\%) of all attention to the first key
(as in \cref{ssec:pd-first-token}, evaluation is performed on the validation set of the \texttt{en} split of the C4 dataset).
Despite a small reduction in first token dominance, the anomaly persists in the model without positional encodings,
therefore we conclude that the positional encodings are not the cause of the first token dominance in attention maps.

\subsection{Removing First Token Dominance of Attention Maps}\label{ssec:first-token-sol}
In the previous section we eliminated positional encodings as a potential cause of the first token dominance in attention maps.
Some other aspects of Transformer models were dismissed as potential causes of the anomaly due to
their action being invariant to the token position.
We blame a combination of two aspects of Transformer models which lead to first token dominance:
(1) the causal masking of self-attention in language models, and
(2) softmax normalisation of the attention scores.
The causal masking of self-attention (\ie~the masking which prevents tokens from attending to future tokens during training)
is the strictest form of privilege the first token receives in the model.

Consider the self-attention mechanism on the initial token positions in a transformer model with causal masking.
The first query token can only attend to its own key and due to the softmax normalisation, it receives an attention score of 1.
Similarly, the second query token can only attend to its own key and the first key,
and due to the softmax normalisation, the attention scores must sum to 1.
There are many works which demonstrate a given attention head specialises to a particular concept or
group of concepts~\citep{voita2019analyzing,bansal2023rethinking}.
Despite this, when a given input sequence is not relevant to an attention heads' specialisation,
it must still allocate attention summing to 1 (due to the softmax normalisation) and
the causal masking of self-attention privileges the first (key) token above all other tokens as
it is the only key token to which \emph{all} queries can attend (due to the causal masking).
This explains why any particular token position dominates the attention maps and specifically,
why the \emph{first} token dominates the attention maps, rather than any other token position.

Previous works have suggested solutions to the first token dominance in attention maps, such as
adding registers (extra learnt tokens forming part of the input sequence)~\citep{darcet2024vision} or clipping the softmax
function and adding gating to the attention scores~\citep{bondarenko2023removing}.

We propose a much simpler solution to the first token dominance anomaly by simply
modifying the softmax normalisation of the attention scores.

Consider the canoncial softmax function on a logit vector $\mathbf{x} \in \real^L$,
where $L$ is the sequence length:
\begin{align}
    \text{softmax}(x_i) &= \frac{\exp(x_i)}{\sum_{j=1}^{L} \exp(x_j)} \\
    \sum_{i=1}^{L} \text{softmax}(x_i) &= 1
\end{align}
we see that even if logit scores for (query, key) pairs are all small, the softmax normalisation
enforces that the attention scores sum to 1 leading to the first token dominance anomaly.
We propose a simple modification to the softmax function:
\begin{align}
    \text{softmax-1}(x_i) &= \frac{\exp(x_i)}{1 + \sum_{j=1}^{L} \exp(x_j)} \\
    \sum_{i=1}^{L} \text{softmax-1}(x_i) &< 1
\end{align}
where we add a constant 1 to the denominator of the softmax function.
This modification removes the strict normalisation of the attention scores to 1 and allows the model to
allocate attention scores as it sees fit \ie~low logit scores across all (query, key) pairs will result in
low attention scores across all (query, key) pairs.
In the limit of one or more logit scores being very large, the softmax-1 function will approach the canonical softmax function.
Note that we only modify the softmax function in the self-attention mechanism and not in the final language modeling head which predicts the next token
across the model vocabulary.

Looking at this modification from the ``registers'' perspective, the constant 1 in the denominator
of the softmax-1 function can be thought of as a register (key) token which always has logit score 0 with
respect to all queries.

We train a GPT2 model with the softmax-1 function and observe the attention maps,
comparing them to another GPT2 model trained with the canonical softmax function, all other parameters and hyperparameters being the same
(\ie~both models have learnt absolute positional encodings).
We find that the GPT2 model with the softmax-1 (canonical softmax) function exhibits first token dominance in 2\% (53\%) of the (query, head) pairs and
allocates 4\% (46\%) of all allocated attention to the first key.
Note that because of the softmax-1 function, the attention scores are not enforced to sum to 1 and
therefore the \emph{sum of all attention scores across all (query, head) pairs is not the same as that in the model with canonical softmax function}.
We find that the softmax-1 model allocates $\sim$45\% of the attention compared to the canonical softmax model.

Figure xyz shows the average attention maps of our GPT2 models trained with: (1) canonical softmax and learnt position encodings (standard model);
(2) canonical softmax and no positional encodings; and (3) softmax-1 and learnt position encodings.

Importantly, we find the training of the GPT2 model with the softmax-1 function is stable and almost identical to the training of the standard GPT2 model in
terms of convergence and perplexity on the validation set of the C4 dataset
(please see the appendix for comparative training curves between the models mentioned in this section and for details on the training procedure we use).

\subsection{Discussion}\label{ssec:disc-first-token}
We have shown that the first token dominance in attention maps is a result of the causal masking of self-attention,
which privileges the first token position above all other tokens,
combined with the softmax normalisation of the attention scores forcing the total attention allocated in a given (query, head) pair to sum to 1.
Our proposed a simple modification to the softmax function, which removes the strict normalisation of the attention scores to 1,
results in a model which does not demonstrate first token dominance in attention maps.
The softmax-1 function has been mentioned previously in a short blogpost which discusses softmax-1 as the solution to
the \emph{outlier activations in the residual stream} not the first token dominance in attention maps~\citep{miller2023attention}.
Figure xyz shows the mean absolute value of the activations in the hidden states of a GPT2 model trained with the canonical softmax function (with and without positional encodings)
and the softmax-1 function (with positional encodings).
We find that the only significant change in the outlier activations is that the extreme outliers observed in the first token position
of the hidden states of the GPT2 model trained with the canonical softmax function (with or without positional encodings) are no longer present in the GPT2 model trained with the softmax-1 function,
which is intuitive as softmax-1 removes the privilege of the first token position in the attention maps over all other token positions.
However, the general outlier activations in specific feature channels across all token positions remain in the GPT2 model trained with the softmax-1 function.
Therefore, we conclude that the first token dominance in attention maps and the outlier activations in the residual stream are not related and
a separate solution is required to address the latter anomaly.


% Considering a single head of self-attention given hidden states $\mathbf{X} \in \real^{L \times D}$,
% where $L$ is the sequence length and $D$ is the hidden dimension, self-attention in a single head is given by
% \begin{align}
%     \text{Attention}(\mathbf{X}; \mathbf{W}_Q, \mathbf{W}_K, \mathbf{W}_V) = \text{softmax}\left(\frac{\mathbf{Q}\mathbf{K}^T}{\sqrt{D}}\right)\mathbf{V},
% \end{align}



==> sections/05-prelim.tex <==
\section{Outlier Activations: Preliminaries}\label{sec:prelim}

Previous sections have introduced the presence of large outlier activations in the
hidden states/residual stream of transformer models.
While visual representations of these outliers are useful for illustrating the issue
(such as in~\cref{fig:teaser_hs}(top)),
more quantitative measures are needed to understand the extent of the problem and to track
the effectiveness of our proposed solution.

To establish the extent of outliers in the hidden states of transformer models,
we use kurtosis as a measure of the tail heaviness of the distribution.
Noting that the kurtosis of a Gaussian distribution is 3,
we use 3 as a target value for the kurtosis of the hidden states.
Values of kurtosis greater than 3 indicate heavier tails than a Gaussian distribution
(\eg~the exponential distribution has a kurtosis of 6) and values less than 3 indicate lighter tails
(\eg~the uniform distribution has a kurtosis of 1.8).
Given hidden states $\mathbf{X} \in \mathbb{R}^{M \times L \times D}$ of a transformer model,
where $M$ is the number of layers, $L$ is the number of tokens and $D$ is the number of feature channels,
the per-layer, per-position kurtosis of the hidden states is computed as:
\begin{align}
    \kappa_{m,l} = \text{Kurt}_{m,l}\left[X_{m,l,d}\right] = \frac{\expect_{d}[(X_{m,l,d} - \mu_{m,l})^4]}{\expect_{d}[(X_{m,l,d} - \mu_{m,l})^2]^2},
        \quad \text{where} \quad \mu_{m,l} = \expect_{d}[\mathbf{X}_{m,l,d}] % \label{eq:kurt-layer} \\
    % \text{Kurt}(\mathbf{X}_{l}) &= \frac{\expect_{m,d}[(\mathbf{X}_{m,l,d} - \mu_{l})^4]}{\expect_{m,d}[(\mathbf{X}_{m,l,d} - \mu_{l})^2]^2},
    %     \quad \text{where} \quad \mu_{l} = \expect_{m,d}[\mathbf{X}_{m,l,d}] \label{eq:kurt-position} \\
    % \text{Kurt}(\mathbf{X}) &= \frac{\expect_{m,l,d}[(\mathbf{X}_{m,l,d} - \mu)^4]}{\expect_{m,l,d}[(\mathbf{X}_{m,l,d} - \mu)^2]^2},
    %     \quad \text{where} \quad \mu = \expect_{m,l,d}[\mathbf{X}_{m,l,d}] \label{eq:kurt-overall}
\end{align}
where $X_{m,l,d}$ is the hidden state in layer $m$ at position $l$ for feature $d$,
and $\mu_{m,l}$ is the mean hidden state value of the hidden states in layer $m$ at position $l$.

In this work, we shall use kurtosis of the hidden states to measure
the presence of activation outliers.
Specifically, given first token dominance cause \emph{even more extreme} outliers in the hidden states of the first token,
we shall separate the kurtosis of the hidden states between the first token, $\kappa_{m,1}$, and the rest of the tokens, $\kappa_{m,l}$ for $l > 1$.
In~\cref{sec:exp}, where we present our experimental results, we shall give averages of these two kurtosis values across all layers.
\prannay{The appendix presents more granular results showing the change in kurtosis across layers of transformer models.}

==> sections/06-oa.tex <==
\section{Method: Outlier Activations}\label{sec:oa}

\Cref{fig:teaser_hs}(top) shows the presence of large outlier activations in the hidden states of a transformer model.
In this section, we explain what kinds of operations could lead to the presence of these outliers,
eliminate certain causes and propose a novel solution to address the issue.

Outlier activations in consistent and particular feature channels of the hidden states in the residual stream indicate
that some operation which which operates in the basis of the residual stream is causing the issue.

Starting from the original GPT2 model, we will eliminate particular plausible causes of the outlier activations
empirically and show that the issue persists.

\parb{Attention and MLP Output Biases}
A plausible cause of the outlier activations in the hidden states of the GPT2 model is the presence of biases in the attention and MLP output layers.
However, Llama models, which do not have biases in the attention and MLP output layers, also exhibit the same outlier activations.
Therefore, it is unlikely that the biases in the attention and MLP output layers are the cause of the outlier activations,
but given biases are applied in the same basis as the residual stream, we remove them from the model to investigate further.

\parb{Normalisation Layers}
Another plausible cause of the outlier activations in the hidden states of the GPT2 model is the presence of normalisation layers.
GPT2 models use LayerNorm~\citep{ba2016layer}, which subtracts the mean and divides by the standard deviation of the hidden states along the feature channels.
Additionally, a per-channel affine transformation is applied after normalisation.
The mean subtraction and the \emph{per-channel} affine transformation both operate in the basis of the residual stream,
and so could potentially cause the outlier activations.
Llama models, use RMSNorm~\citep{zhang2019root}, which divides by the root mean square of the hidden states along the feature channels
and applies a per-channel \emph{scaling}.
This scaling operation also operates in the basis of the residual stream and so could potentially cause the outlier activations.
To remove the effect of the normalisation layers, we replace LayerNorm in our trained GPT2 models with
a version of RMSNorm which applies a global scale instead of a per-channel scaling---``RMSNormSingle''.

We find that the outlier activations persist in the hidden states of a GPT2 model trained without biases and with RMSNormSingle.
\Cref{tab:ablation_big} shows the kurtosis of the hidden states remains high in models trained without biases and/or with RMSNormSingle.

\parb{Optimizer Selection}
Another potential cause of outlier activations is the optimizer.
Most transformer models are trained with the Adam optimizer~\citep{kingma2015adam} or some variant of it (Llama models use AdamW~\citep{loshchilov2019decoupled}).
These optimizers calculate the first and second moments of the gradients using exponential moving averages
and use them to update the model parameters.
Rather than per-channel operations (like normalisation layers), the optimizer tracks these moments at a parameter level.
The key hyperparameters of Adam optimizers (other than the learning rate) are $\beta_1$ and $\beta_2$,
which control the decay rates of the first and second moments respectively.
If $\beta_2 = 0$, the optimizer only tracks the first moment of the gradients and resembles stocastic gradient descent with momentum.
Conversely, if $\beta_1 = 0$, the optimizer only tracks the second moment of the gradients and resembles RMSProp.

To investigate the effect of the optimizer on the outlier activations we train a series of GPT2 models using the different optimizers
to account for the effect of each of the moments on outlier activations.
We train 4 models as follows:
(1) default Adam;
(2) RMSProp (Adam with $\beta_1 = 0$);
(3) SGD with momentum; and
(4) SGD without momentum.
These experiments require tuning of the learning rate to ensure successful training, these details are provided in the appendix.\prannay{update}
Expectedly, the models trained with SGD without momentum converges the slowest and has the largest validation perplexity,
whereas the model trained with Adam converges the fastest and has the smallest validation perplexity.
However, we find that while models (1)-(2) have high kurtosis values in the hidden states,
model (3) has a kurtosis value of $\sim$5.0 and
models (4) has a kurtosis value of $\sim$3.0.
These results are shown in our ablation study (\cref{ssec:ablation}).
This suggests that the optimizer is a key factor in the presence of outlier activations.

This finding leaves us with a key practical question for training transformer models:
``How can we train a model with an optimizer that has the speed and convergence properties of Adam,
but produces activations properties similar to SGD without momentum''?

\subsection{OrthoAdam}\label{ssec:orthoadam}
From the experiments described above, we find that optimizers which track exponential decaying averages of the
first and/or second moments of the gradients lead to outlier activations in the hidden states of transformer models.
We note that the optimizer calculates these gradient averages in the same basis as the parameters of the model.
Moreover, in the models trained above, the largest absolute \emph{parameter} values correspond to the features
which exhibit the largest outlier activations in the hidden states/residual stream \ie~if outlier activations occur
in feature channel $d$ of the residual stream,
the largest absolute parameter values correspond to specific weights of the model which contribute to
feature channel $d$ of the residual stream \eg~output projection weights of the attention and MLP layers.
\prannay{some more on this}
Therefore, to arrive at these large parameter, which contribute to outlier activations, the optimizer (\eg~Adam) must
provide large updates to these specific parameters and not others.
An idealised case of this issue is addressed below using orthogonal transformations, which inspire our proposed solution
to the outlier activation problem.

%give an illustration that rotating a heavily skewed parameter with a random orthogonal matrix can lead to a more balanced parameter.
Consider a $D$-dimensional vector which has all its mass in one direction---$\mathbf{x} = \alpha \mathbf{e}_i$,
where $\mathbf{e}_i$ is the $i$th unit vector in the standard basis, $\mathbf{x} \in \real^D$ and $\alpha \in \real$.
This vector is heavily skewed and has high kurtosis and represents an illustration of the outlier activations
we observe in the hidden states of transformer models.
We find that for large $D$, $\text{Kurt}[{\mathbf{x}}] \propto D$, and so we
expect larger transformer models to have larger activation kurtosis.

In the above example, we have taken the extreme case of a vector with all its mass in one direction as a proxy for what we
in transformer models. Note that in this idealised case of high kurtosis,
the ratio $\frac{\left\lVert\mathbf{x}\right\rVert_{\infty}}{\left\lVert\mathbf{x}\right\rVert_{2}} = 1$.
The corrollary being that features in which the $\ell_\infty$-norm is close
to $\ell_2$-norm are those which must have high kurtosis for large $D$.
(The converse is not necessarily true.)
We observe this in the hidden states of transformer models---in the middle layers of a GPT2-Medium model, where $D=1024$,
$\frac{\left\lVert\cdot\right\rVert_{\infty}}{\left\lVert\cdot\right\rVert_{2}} \approx 0.97$. \prannay{see appendix}
Noting that transforming the basis of a vector through an orthogonal matrix, $\mathbf{Q}$,
does not change the $\ell_2$-norm of the transformed vector \prannay{(see appendix)},
we can use an orthogonal transformation of $\mathbf{x}$ to reduce 
$\frac{\left\lVert\mathbf{x}\right\rVert_{\infty}}{\left\lVert\mathbf{x}\right\rVert_{2}}$ and consequently the
kurtosis---note weight decay used during training generally utilises $\ell_2$-norm regularisation to prevent large weights.
In this idealised case, a transformed vector, $\mathbf{y} = \mathbf{Q}\mathbf{x}$,
has minimal $\ell_\infty$-norm when all the elements of $\mathbf{y}$ are equal in magnitude
and $\frac{\left\lVert\mathbf{x}\right\rVert_{\infty}}{\left\lVert\mathbf{x}\right\rVert_{2}} = \frac{1}{\sqrt{D}}$.
\prannay{see appendix}

The above example illustrates how applying an orthogonal transformation to a vector can reduce the $\ell_\infty$--norm of the vector.
We now apply this concept to the gradient updates of the parameters of a model which occur in an optimizer during training.
In Adam optimizers and similar (\ie~those optimizers in which $\beta_1$ and/or $\beta_2$ are non-zero),
we have gradient updates which are analogous to the vector $\mathbf{x}$ above leading to large parameter values in specific feature dimensions,
which cause outlier activations in the hidden states of transformer models.
\prannay{see appendix for evidence of this}
We propose a novel optimizer, \emph{OrthoAdam}, in which the gradient updates are computed under an orthogonal
transformation---analogous to creating the vector $\mathbf{y}$ using $\mathbf{Q}$ above.

We propose a novel optimizer, OrthoAdam, which tracks the first and second moments of the gradients for a given parameter,
but applies a unique (\wrt~other parameters) orthogonal transformation to the gradients before calculating first and second moments.

%Adam Algorithm
\setlength\fboxsep{1.00pt}
\begin{algorithm}[tb!]
\caption{OrthoAdam.\prannay{update} $\mathbf{\bar{g}}^2_t$ is the element-wise square $\mathbf{\bar{g}}_t \odot \mathbf{\bar{g}}_t$.
         With $\beta_1^t$ and $\beta_2^t$ we mean $\beta_1$ and $\beta_2$ taken to the power of $t$.}
\footnotesize
\label{algo_adam}
\begin{algorithmic}
\STATE{\textbf{given} learning rate: $\eta=0.001$, first moment decay rate: $\beta_1=0.9$, second moment decay rate: $\beta_2=0.999$,
       numerical epsilon: $\epsilon=10^{-8}$}\label{adam-Given}
\STATE{\textbf{initialize} time step: $t \leftarrow 0$, parameter vector: $\mathbf{\theta}_{t=0} \in \R^n$,  first moment vector: $\mathbf{\bar{m}}_{t=0} \leftarrow \mathbf{0}$,
       second moment vector: $\mathbf{\bar{v}}_{t=0} \leftarrow \mathbf{0}$, schedule multiplier: $\lambda_{t=0} \in \R$,
       \orthoadamtext{unique orthogonal matrix: $\mathbf{Q} \in \mathcal{O}^n$}}\label{adam-Init}
\REPEAT{}
	\STATE{$t \leftarrow t + 1$}
	\STATE{$\nabla f_t(\mathbf{\theta}_{t-1}) \leftarrow  \text{SelectBatch}(\mathbf{\theta}_{t-1})$}\COMMENT{select batch and calculate gradient}
	\STATE{$\mathbf{g}_t \leftarrow \nabla f_t(\mathbf{\theta}_{t-1})$}\COMMENT{store the gradient in model parameter basis}
    \STATE{\orthoadamtext{$\mathbf{\bar{g}_t} \leftarrow \text{MatMul}(\mathbf{Q},\mathbf{g}_t$)}}\COMMENT{transform gradient into unique optimizer basis}
	\STATE{$\mathbf{\bar{m}}_t \leftarrow \beta_1 \mathbf{\bar{m}}_{t-1} + (1 - \beta_1) \mathbf{\bar{g}}_t$}\COMMENT{update biased first moment estimate}\label{adam-mom1} 
	\STATE{$\mathbf{\bar{v}}_t \leftarrow \beta_2 \mathbf{\bar{v}}_{t-1} + (1 - \beta_2) \mathbf{\bar{g}}^2_t$}\COMMENT{update biased second raw moment estimate}\label{adam-mom2} 
	\STATE{$\mathbf{\hat{m}}_t \leftarrow \mathbf{\bar{m}}_t/(1 - \beta_1^t)$}\COMMENT{compute bias-corrected first moment estimate}\label{adam-corr1}
	\STATE{$\mathbf{\hat{v}}_t \leftarrow \mathbf{\bar{v}}_t/(1 - \beta_2^t)$}\COMMENT{compute bias-corrected second raw moment estimate}\label{adam-corr2}
    \STATE{$\mathbf{\bar{s}}_t \leftarrow \hat{\mathbf{m}}_t / (\sqrt{\hat{\mathbf{v}}_t} + \epsilon)$}\COMMENT{calculate the update step in unique optimizer basis}
    \STATE{\orthoadamtext{$\mathbf{s}_t \leftarrow \text{MatMul}(\mathbf{Q}^T,\mathbf{\bar{s}})$}} \COMMENT{transform the update step back to model parameter basis}
	\STATE{$\lambda_t \leftarrow \text{SetScheduleMultiplier}(t)$}	\COMMENT{can be fixed, decay, or also be used for warm restarts}
    \STATE{$\mathbf{\theta}_t \leftarrow \mathbf{\theta}_{t-1} - \lambda_t \mathbf{s}_t$}\COMMENT{apply parameter update}\label{adam-xupdate}
\UNTIL{\emph{stopping criterion is met}}
\RETURN{optimized parameters $\mathbf{\theta}_t$}
\end{algorithmic}
\end{algorithm}
\setlength\fboxsep{4pt}

In our experiments we randomly sample the orthogonal matrix for each parameter (which remains fixed during the training of the model).
We find that using OrthoAdam---which is a drop-in replacement for Adam---leads to a significant reduction in the kurtosis of hidden states
in transformer models, effectively eliminating the outlier activations.
This is shown in~\cref{fig:teaser_hs}(bottom), where feature channels with high absolute activation values in the hidden states
across all token positions \emph{are no longer present}.
\prannay{see appendix}.







==> sections/09-ack.tex <==
\subsubsection*{Acknowledgments}
Blah
